LOVE: Benchmarking and Evaluating Text-to-Video Generation and Video-to-Text Interpretation

Recent advancements in large multimodal models (LMMs) have driven substantial progress in both text-to-video (T2V) generation and video-to-text (V2T) interpretation tasks. However, current AI-generated videos (AIGVs) still exhibit limitations in terms of perceptual quality and text-video alignment. Therefore, a reliable and scalable automatic model for AIGV evaluation is desirable, which heavily relies on the scale and quality of human annotations. To this end, we present AIGVE-60K, a comprehensive dataset and benchmark for AI-Generated Video Evaluation, which features (i) comprehensive tasks, encompassing 3,050 extensive prompts across 20 fine-grained task dimensions, (ii) the largest human annotations, including 120K mean-opinion scores (MOSs) and 60K question-answering (QA) pairs annotated on 58,500 videos generated from 30 T2V models, and (iii) bidirectional benchmarking and evaluating for both T2V generation and V2T interpretation capabilities. Based on AIGVE-60K, we propose LOVE, a LMM-based metric for AIGV Evaluation from multiple dimensions including perceptual preference, text-video correspondence, and task-specific accuracy in terms of both instance level and model level. Comprehensive experiments demonstrate that LOVE not only achieves state-of-the-art performance on the AIGVE-60K dataset, but also generalizes effectively to a wide range of other AIGV evaluation benchmarks. These findings highlight the significance of the AIGVE-60K dataset. Database and codes are anonymously available at https://github.com/IntMeGroup/LOVE.

==> tables/cross2.tex <==
\begin{table*}[!h]
  \centering
  % \vspace{-3mm}
    \caption{Zero-shot cross-dataset performance comparison on multiple benchmarks. *Refers to scores finetuned on the specific dataset.} %*refers to finetuned scores. }
  \label{tab:method}%
 
  \renewcommand\arraystretch{0.98}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc}
    \Xhline{1px}
    \multirow{2}[1]{*}{Method}& \multicolumn{2}{c|}{\textbf{AIGVE-60K}} & \multicolumn{2}{c|}{FETV} & \multicolumn{2}{c|}{T2VQA-DB} & \multicolumn{2}{c|}{LGVQ} & \multicolumn{2}{c|}{MQT} & \multicolumn{2}{c|}{AIGVQA-DB} & \multicolumn{2}{c|}{GenAI-Bench} \\
\cline{2-15}     & SRCC  & KRCC & SRCC  & KRCC  & SRCC  & KRCC  & SRCC  & KRCC  & SRCC  & KRCC & SRCC  & KRCC & SRCC  & KRCC \\
    \hline
    CLIPScore~\cite{hessel2021clipscore} & 0.095 &  0.064 & 0.607 & 0.498 & 0.049 & 0.033 & 0.446 & 0.301 & 0.772 & 0.611 & 0.152 & 0.101 & 0.536 & 0.180\\
    BLIPScore~\cite{li2022blip} &0.188  &  0.127 & 0.616 & 0.505 & 0.174 & 0.118 & 0.455 & 0.319 &  0.761  & 0.616 & 0.181 & 0.122 & 0.546 & 0.201\\
    ImageReward~\cite{xu2023imagereward} & 0.418 & 0.288 & 0.657 & 0.519 & 0.175  & 0.119 & 0.498 & 0.344 & 0.794 & 0.624 & 0.231 & 0.157 & 0.600 & 0.314\\
    PickScore~\cite{kirstain2023pick} & 0.403 & 0.276 & 0.669 & 0.533 & 0. & 0. & 0.501 & 0.353 & 0.823 & 0.649 & 0. & 0. & 0.568 & 0.248\\
    HPSv2~\cite{wu2023human} & 0.542 & 0.379 & 0.686 & 0.540 & 0. & 0. & 0.504 & 0.357 & 0.819 & 0.643 & 0. & 0. & 0.515 & 0.137 \\
    VQAScore~\cite{li2024evaluating} & 0.168 & 0.110 & 0.565 & 0.414 & 0.177 & 0.121 & 0.553 & 0.394 & 0.492 & 0.341 & 0.444 & 0.307 & 0.632 & 0.382 \\
    \hline
 %    FGA-BLIP2 (w/o var, os) & 0.7708 & 0.7698 & 0.5548 & 0.5589 & 0.7548 & 0.741 & 0.5073 & 0.5384 \\
 % FGA-BLIP2 (es\_avg) & 0.6809 & 0.6867 & 0.5206 & 0.5259 & 0.7419 & 0.736 & 0.3413 &0.3096 \\
    % FGA-BLIP2 (os) & 0.7742} & 0.7722} & 0.5637 & 0.5673 & 0.7604 & 0.7442 & 0.5123} & 0.5455} \\
    % FGA-BLIP2~\cite{han2024evalmuse40kreliablefinegrainedbenchmark} & 0.518 & 0.361 &  \\
    % \hline
    \rowcolor{gray!20} LOVE (Ours)  & & &0.724 & 0.555 \\
     % \rowcolor{gray!20}Ours (Train on EvalMuse) &  \textbf{\blue{0.6764}} & \textbf{\blue{0.6928}}  & \textbf{\red{0.7852*}}  & \textbf{\red{0.7958*}}  & \textbf{\blue{0.6523}} & \textbf{\blue{0.6363}} &  0.7390 & 0.7264 & \textbf{\blue{0.5836}} & \textbf{\blue{0.5972}} & \textbf{\blue{0.7797}} & \textbf{\blue{0.8118}} & 0.6823 & 0.6782  \\
    % EvalMi (Ours) 26B&   \\
%     \rowcolor{gray!20}\textit{Improvement} 

% & +2.7\% & +3.0\% &+ 5.7\%  

% & +1.7\% & +0.2\% &+8.5\%  \\
    \Xhline{1px}
    \end{tabular}%
  }
\end{table*}%
% \vspace{-9mm}

==> tables/tasks.tex <==
\begin{table*}[tbph]
\vspace{-13mm}
\setlength{\belowcaptionskip}{-0.01cm}
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\renewcommand\arraystretch{0.87}
\caption{Performance comparisons of LMMs on the AIGVE-60K across different task-specific challenges. We report the correlation between automatic evaluation metrics and human groundtruth annotations in terms of perception quality SRCC ($\rho_p$), correspondence SRCC ($\rho_c$), and QA accuracy (Acc\%). 
The best results are marked in {\textcolor{red}{RED}} and the second-best in {\blue{BLUE}}. 
*Refers to finetuned 
}

   

     \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{Object}}&\multicolumn{3}{c}{\textbf{Color}}&\multicolumn{3}{c}{\textbf{Counting}}&\multicolumn{3}{c}{\textbf{Texture}}&\multicolumn{3}{c}{\textbf{Position}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 Methods / Metrics
&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.048 & 0.027 &33.33&0.003&0.025&25.00&0.018&0.004&50.00 &0.032 &0.004 &36.36 &0.042 &0.015 &80.00\\
     VideoLlava (7B)~\cite{liu2024improved} &0.193&0.198 &72.22& 0.108&0.381&70.00&0.185 &0.163& 60.00 &0.411 &0.310 &63.64 & 0.040 &0.383 &70.00\\
    mPLUG-Owl3 (7B)~\cite{ye2024mplug} &0.316 &0.504&77.78& 0.392 &0.535&70.00& 0.333 &0.641 &50.00 &0.318 &0.666&81.82 &0.293 & 0.720 & 80.00\\ 
   VideoLlama3 (8B)~\cite{yao2024minicpm}&0.365 &0.381 &83.33& 0.391 &0.488&70.00& 0.498 &0.466& 40.00&0.346&0.394& 72.73 &0.406 &0.573 &70.00\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}&0.506&0.497 &72.22& 0.500 &0.538 &65.00&0.616 &0.455& 60.00&0.653 &0.717&81.82 &0.592 &0.722 &80.00\\
    Llama3.2-Vision (11B)~\cite{meta2024llama}
    &0.027 &0.055&72.22&0.094 &0.181&55.00&0.107 &0.108& 80.00 &0.113 &0.164 &63.64 & 0.267 &0.020 &90.00\\
  CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}&0.150 &0.130 &77.78&0.167 &0.185&70.00& 0.117 & 0.165 &50.00 &0.060 &0.169 &72.73 &0.106 & 0.127 &50.00\\
  % InternVL2 (8B)~\cite{wang2024mpo}& 0.1230 & 0.3695  & 0.8345 & 0.1447 & 0.6436 & 0.8229 & 0.0701 & 0.5815 & 0.7136 & 0.0890 & 0.5478 & 0.8652 & 0.1585 & 0.6041  & 0.5412 & 0.0982 & 0.4042 & 0.6393 & 0.1226 & 0.5715 & 0.7232\\
    InternVL2.5 (8B)~\cite{chen2024expanding}&0.309 &0.448 &83.33& 0.258 &0.543& 65.00&0.366&0.507& 60.00&0.330 &0.590&63.64 &0.307 &0.628 &70.00 \\
    InternVL3 (9B)~\cite{chen2024expanding}&0.229 &0.467 &83.33& 0.257 &0.441 &60.00&0.298 &0.536 &40.00 &0.371 &0.566 &90.91 &0.310 &0.632 &50.00\\
   InternVideo2.5 (8B)~\cite{internlmxcomposer}&0.235 &0.529  &83.33&0.101 &0.545&75.00&0.298 &0.606&50.00 &0.125 &0.555&63.64  &0.088 &0.766 &70.00\\
   LLaVA-NeXT-Video (8B)~\cite{liu2024llavanext} & 0.463 &0.357&72.22& 0.421&0.380&75.00& 0.613 &0.313 &60.00 &0.551 &0.353& 54.55 &0.567 &0.423 &80.00\\
    % Llava-Onevision (0.5B)~\cite{li2024llava}& 0.1099 & 0.2670 & 0.7692 & 0.0068 & 0.3457 & 0.6057 & 0.0605 & 0.2331 & 0.7591 & 0.0460 & 0.1960 & 0.8571 & 0.0865 & 0.1988 & 0.7228 & 0.2047 & 0.2224 & 0.5871 & 0.0685 & 0.2074 & 0.6808\\
    \hdashline
   ChatGPT-4o &0.403 &0.622 &77.78&0.455 &0.655 &70.00& 0.681 &0.757 &70.00&0.652 &0.748 &81.82&0.682&0.813&90.00\\
   Gemini Pro Vision &0.494 & 0.611 &77.78&0.418 &0.630 &70.00&0.611 &0.668&60.00&0.532 &0.680&72.73&0.585&0.763&80.00\\
   Claude 3 & 0.362 &0.594 & 77.78&0.401 &0.618 & 65.00& 0.516 &0.576 & 60.00&0.517 &0.705 &72.73&0.488 &0.689&70.00\\

   Grok &0.488 &0.641&77.78&0.501&0.697&70.00&0.653&0.737&60.00&0.649&0.739&90.91&0.552&0.793&80.00\\
   \hline
   % *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}&  \\
   *InternVL3 (9B)~\cite{meta2024llama}& 0.630 & 0.614 & 72.22&0.596 &0.535 &60.00&0.681 &0.711 &70.00&0.704 &0.715 &72.73&0.692 &0.738&60.00\\

   *InternVideo2.5 (8B)& 0.799 &0.708 &83.33&0.741 &0.713 &75.00& 0.832 &0.736 &60.00&0.828 &0.748&72.73&0.871&0.856&80.00\\
   
   \rowcolor{gray!20} \textbf{LOVE (Ours)} &0.786&0.747&77.78&0.745&0.754&60.00&0.837&0.808&50.00&0.871&0.845&72.73&0.847&0.862&60.00\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}


     \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{HOI}}&\multicolumn{3}{c}{\textbf{Face}}&\multicolumn{3}{c}{\textbf{Emotion}}&\multicolumn{3}{c}{\textbf{Human}}&\multicolumn{3}{c}{\textbf{OCR}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 Methods / Metrics
&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.004 &0.029 & 20.00 & 0.077 &0.075 &41.67 &0.006 &0.112 & 33.33 & 0.034 & 0.098 & 40.00 & 0.063 &0.087 & 75.00 \\
     VideoLlava (7B)~\cite{liu2024improved} & 0.175 &0.338  & 86.67  &0.146 &0.360  & 58.33 & 0.118  &0.244 &66.67& 0.129 & 0.200 & 90.00 & 0.140 & 0.057 & 75.00 \\
    mPLUG-Owl3 (7B)~\cite{ye2024mplug} &  0.453 &0.590 & 60.00 &0.313 &0.539 & 66.67 & 0.366 &0.478 & 55.56 & 0.365 &0.483 & 80.00 & 0.334 & 0.675 & 91.67  \\ 
   VideoLlama3 (8B)~\cite{yao2024minicpm}& 0.424 &0.509 &  63.33 & 0.335 &0.389 & 58.33 & 0.179 &0.330 &66.67& 0.507 &0.397 & 80.00 & 0.287 & 0.400 & 100.0 \\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.560 &0.492 & 36.67 & 0.630 &0.475 & 58.33 & 0.537 & 0.232 & 66.67 & 0.543 & 0.442 & 70.00 & 0.433 &0.640 & 91.67 \\
    Llama3.2-Vision (11B)~\cite{meta2024llama}
    & 0.067 & 0.028 & 63.33 & 0.056 &0.003 & 75.00 & 0.116 &0.090 & 44.44 & 0.072 & 0.009 & 70.00 & 0.120 & 0.117 & 91.67 \\
    % DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1875 &0.0224 &0.4406 &0.2191 &0.0916 &0.4495 &0.2312 &0.0164&0.5545 &0.1640 &0.0824 &0.3260 &0.1701 &0.0555 &0.4757 &0.3304 &0.0453 &0.5050 & 0.2160 & 0.0549 & 0.5781\\
  CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.107 &0.108 & 80.00& 0.231 &0.157 & 66.67 &0.096 &0.079 & 66.67 &0.089 &0.122 & 80.00 & 0.123 & 0.125 & 41.67 \\
  % InternVL2 (8B)~\cite{wang2024mpo}& 0.1230 & 0.3695  & 0.8345 & 0.1447 & 0.6436 & 0.8229 & 0.0701 & 0.5815 & 0.7136 & 0.0890 & 0.5478 & 0.8652 & 0.1585 & 0.6041  & 0.5412 & 0.0982 & 0.4042 & 0.6393 & 0.1226 & 0.5715 & 0.7232\\
    InternVL2.5 (8B)~\cite{chen2024expanding}& 0.299 &0.452 & 80.00 &0.187 &0.276 & 66.67 & 0.175 &0.320 & 66.67 & 0.339  &0.459 & 70.00 & 0.180 & 0.561 & 91.67  \\
    InternVL3 (9B)~\cite{chen2024expanding}&0.293 &0.482 &70.00 & 0.348 &0.359 &66.67 &0.289 &0.448 &66.67 &0.266 &0.454 & 90.00 & 0.205 & 0.552 & 33.33  \\
    
   InternVideo2.5 (8B)~\cite{internlmxcomposer}& 0.320 &0.496 & 63.33 & 0.200 &0.371 & 66.67 & 0.207 & 0.371 & 55.56 & 0.278 & 0.363 & 100.0 & 0.070 &0.574 & 91.67  \\
   LLaVA-NeXT-Video (8B)~\cite{liu2024llavanext} & 0.532 &0.357 & 73.33 & 0.442 &0.376 & 66.67 &0.474 &0.136 &66.67& 0.501 & 0.325 & 70.00 & 0.525 & 0.120 & 91.67 \\
    % Llava-Onevision (0.5B)~\cite{li2024llava}& 0.1099 & 0.2670 & 0.7692 & 0.0068 & 0.3457 & 0.6057 & 0.0605 & 0.2331 & 0.7591 & 0.0460 & 0.1960 & 0.8571 & 0.0865 & 0.1988 & 0.7228 & 0.2047 & 0.2224 & 0.5871 & 0.0685 & 0.2074 & 0.6808\\
    \hdashline
   ChatGPT-4o&0.564 &0.654&73.33&0.581 &0.659 &58.33&0.523&0.551&55.56&0.577&0.648&80.00&0.706&0.736&91.67\\
   Gemini Pro Vision&0.622 &0.588&77.78&0.566 &0.566&66.67&0.430&0.532&66.67&0.502&0.534&80.00&0.391&0.696&91.67\\
   Claude 3&0.462 &0.607&83.33&0.402&0.486&66.67&0.316&0.443&66.67&0.496&0.519&80.00&0.451&0.649&91.67\\
   Grok & 0.643 &0.655 &83.33&0.629 &0.633 &66.67&0.518&0.577&55.56&0.591&0.652&90.00&0.506&0.755&91.67\\
   \hline
   
   % *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.772} & \bf\blue{0.658}& 89.1 &\bf\blue{0.784} &0.825 &87.8 &\bf\blue{0.766} &\bf\blue{0.820}& 86.9 &\bf\blue{0.774} & \bf\blue{75.1} &\bf\blue{89.5} &\bf\blue{0.795} & 0.604 & \\
   % *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& \\
   *InternVL3 (9B)~\cite{meta2024llama}& 0.660 &0.597 &63.33&0.763&0.531&58.33&0.665&0.444&66.67&0.652&0.572&90.00&0.630&0.744&91.67\\
   *InternVideo2.5 (8B)& 0.833 &0.692 &63.33&0.853&0.744 &75.00&0.789&0.569&66.67&0.791&0.648&80.00&0.818&0.864&91.67\\
   
   \rowcolor{gray!20} \textbf{LOVE (Ours)} &0.822&0.749&70.00&0.877&0.773&75.00&0.804&0.651&66.67&0.790&0.671&90.00&0.856&0.806&91.67\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
  

     \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{Scene}}&\multicolumn{3}{c}{\textbf{Style}}&\multicolumn{3}{c}{\textbf{Shape}}&\multicolumn{3}{c}{\textbf{View}}&\multicolumn{3}{c}{\textbf{World Knowledge}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 Methods / Metrics
&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.001 & 0.055 & 22.22 &0.052 &0.004 & 50.00 &0.026 &0.078 & 63.64& 0.108 & 0.045 & 11.11 & 0.005 & 0.119&27.27\\
     VideoLlava (7B)~\cite{liu2024improved} & 0.152 & 0.159 & 66.67 & 0.418 &0.404 & 50.00 & 0.293 &0.244 & 36.36 & 0.233 &0.228 & 88.89 & 0.180 &0.279 & 72.73\\
    mPLUG-Owl3 (7B)~\cite{ye2024mplug} & 0.353 & 0.407 & 74.07 & 0.353 &0.531 & 60.00 & 0.233 & 0.577 & 72.73 &0.358 &0.549 & 77.78 & 0.330 & 0.393 &54.55 \\ 
   VideoLlama3 (8B)~\cite{yao2024minicpm}& 0.466 &0.291 & 74.07 & 0.481 & 0.448 & 40.00 & 0.381 & 0.463 & 54.55 & 0.438 & 0.327 & 83.33 & 0.280 &0.254 & 54.55\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.489 & 0.407 & 55.56 & 0.546 & 0.495 & 70.00 & 0.608 &0.624 & 90.91 & 0.487 &0.412 & 55.56 & 0.494 &0.402 & 45.45 \\
    Llama3.2-Vision (11B)~\cite{meta2024llama}& 0.144  & 0.038& 70.37 & 0.205 &0.156 & 40.00 & 0.215 & 0.154 & 63.64& 0.086 &0.037& 61.11 & 0.056 &0.214 &36.36 \\
    % DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1875 &0.0224 &0.4406 &0.2191 &0.0916 &0.4495 &0.2312 &0.0164&0.5545 &0.1640 &0.0824 &0.3260 &0.1701 &0.0555 &0.4757 &0.3304 &0.0453 &0.5050 & 0.2160 & 0.0549 & 0.5781\\
  CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}&  0.094 &0.080 & 62.96 & 0.259 &0.074 & 30.00 & 0.158 & 0.175 & 63.64& 0.101 &0.130 & 66.67 & 0.127 &0.075 &63.64\\
  % InternVL2 (8B)~\cite{wang2024mpo}& 0.1230 & 0.3695  & 0.8345 & 0.1447 & 0.6436 & 0.8229 & 0.0701 & 0.5815 & 0.7136 & 0.0890 & 0.5478 & 0.8652 & 0.1585 & 0.6041  & 0.5412 & 0.0982 & 0.4042 & 0.6393 & 0.1226 & 0.5715 & 0.7232\\
    InternVL2.5 (8B)~\cite{chen2024expanding}& 0.310 & 0.398 & 74.07 & 0.423 &0.469 &  74.07 & 0.215 &0.481 & 27.27 & 0.255 &0.340 & 72.22 & 0.228 &0.388 & 36.36 \\
    InternVL3 (9B)~\cite{chen2024expanding} & 0.275 &0.380 & 81.48 & 0.300 & 0.395 & 30.00 & 0.314 &0.458 & 72.73 & 0.251 & 0.391 & 72.22 & 0.259 &0.381 & 45.45 \\
   InternVideo2.5 (8B)~\cite{internlmxcomposer}& 0.224 & 0.399 & 77.78 & 0.159 &0.480 & 60.00 & 0.088 & 0.441 & 45.45 & 0.078 & 0.357 & 77.78 & 0.091 &0.454 & 72.73 \\
   LLaVA-NeXT-Video (8B)~\cite{liu2024llavanext} &  0.495 &0.352 &  62.96 & 0.663 &0.261 & 60.00 & 0.549 &0.255 & 63.64& 0.432 & 0.272 & 77.78 & 0.481 &0.148 &72.73 \\
    % Llava-Onevision (0.5B)~\cite{li2024llava}& 0.1099 & 0.2670 & 0.7692 & 0.0068 & 0.3457 & 0.6057 & 0.0605 & 0.2331 & 0.7591 & 0.0460 & 0.1960 & 0.8571 & 0.0865 & 0.1988 & 0.7228 & 0.2047 & 0.2224 & 0.5871 & 0.0685 & 0.2074 & 0.6808\\
    \hdashline
   ChatGPT-4o&0.473&0.504&74.07&0.545&0.584 &50.00&0.569&0.700&63.64&0.419&0.570&61.11&0.360&0.550&63.64\\
   Gemini Pro Vision&0.497 &0.422&66.67&0.514&0.651&60.00&0.461&0.644&45.45&0.485&0.579&83.33&0.506&0.535&63.64\\
   Claude 3&0.438 &0.530&66.67&0.473&0.621&60.00&0.439&0.631&63.64&0.413&0.531&72.22&0.317&0.474&63.64\\
   Grok & 0.579 &0.571 &77.78&0.604&0.630&60.00&0.579&0.581&54.55&0.567&0.562&77.78&0.535&0.498&63.64\\
   \hline
   
   % *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.772} & \bf\blue{0.658}& 89.1 &\bf\blue{0.784} &0.825 &87.8 &\bf\blue{0.766} &\bf\blue{0.820}& 86.9 &\bf\blue{0.774} & \bf\blue{75.1} &\bf\blue{89.5} &\bf\blue{0.795} & 0.604 & \\
   % *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& \\
   *InternVL3 (9B)~\cite{meta2024llama}&0.671&0.431&74.07& 0.700&0.571&50.00&0.728&0.616&36.36&0.600&0.314&77.78&0.601&0.254&63.64\\
   *InternVideo2.5 (8B)& 0.810 &0.578 &62.96&0.855&0.647&40.00&0.850&0.550&81.82&0.748&0.644&88.89&0.796&0.499&63.64\\
   \rowcolor{gray!20} \textbf{LOVE (Ours)} &0.796&0.629&74.07&0.834 &0.772&40.00&0.873&0.629&45.45&0.763&0.643&88.89&0.776&0.527&63.64\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
  

  \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{Linguistic Structure}}&\multicolumn{3}{c}{\textbf{Imagination}}&\multicolumn{3}{c}{\textbf{Motion Direction}}&\multicolumn{3}{c}{\textbf{Event Order}}&\multicolumn{3}{c}{\textbf{Complex}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 Methods / Metrics
&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.015 & 0.046 & 80.00 &0.017 &0.001 & 20.83 & 0.096 & 0.041 & 47.06 & 0.039 &0.076 & 72.73 & 0.028 & 0.059 & 36.84 \\
     VideoLlava (7B)~\cite{liu2024improved} & 0.316 &0.169 & 50.00 & 0.200 &0.200 & 91.67 & 0.081 &0.098 & 52.94 & 0.151 & 0.046 & 63.64& 0.192 & 123 & 73.68\\
    mPLUG-Owl3 (7B)~\cite{ye2024mplug} & 0.283 & 0.795 & 90.00 & 0.280 & 0.456 & 66.67 & 0.345 &0.341 & 64.71 & 0.366 &0.251 & 81.82 &  0.453 & 0.476 & 47.37 \\ 
   VideoLlama3 (8B)~\cite{yao2024minicpm}  &0.418 & 0.755 & 100.0 & 0.441 &0.398 & 79.17 & 0.406 &0.253 & 47.06 & 0.310 & 0.296 & 72.73 & 0.435 & 0.349 & 78.95\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL} & 0.514 &0.639 & 100.0 & 0.571 &0.477 & 37.50 & 0.540 &0.378 & 47.06 & 0.558 & 0.279 & 81.82 & 0.558 & 0.472 & 36.84 \\
    Llama3.2-Vision (11B)~\cite{meta2024llama} & 0.120 & 0.007 & 60.00 & 0.077 &0.046 & 54.17 & 0.064 & 0.054 &41.18 & 0.107 & 0.033 & 90.91 & 0.076 & 0.098 & 42.11 
    \\
  CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}&0.200 &0.074 & 50.00 & 0.096 &0.116 &83.33 &0.093 &0.004 & 52.94 & 0.167 & 0.174 & 18.18 & 0.114 & 0.070 & 78.95\\
    InternVL2.5 (8B)~\cite{chen2024expanding} & 0.320 & 0.603 & 80.00 & 0.288 &0.449 & 79.17 & 0.304 &0.357 & 52.94 & 0.319 & 0.346 &  90.91 & 0.261 & 0.403 & 68.42 \\
    InternVL3 (9B)~\cite{chen2024expanding} &0.244 &0.642 & 80.00 & 0.322 &0.440 & 79.17 & 0.218 & 0.362 &47.06 &0.246 & 0.382 & 27.27 & 0.281 & 0.390 & 84.21 \\
   InternVideo2.5 (8B)~\cite{internlmxcomposer} &0.218 &0.725 & 90.00 & 0.247 &0.438 & 83.33 & 0.113 &0.384 & 41.18 & 0.242 & 0.421 & 72.73 & 0.214 & 0.443 & 73.68 \\
   LLaVA-NeXT-Video (8B)~\cite{liu2024llavanext} &0.487 &0.160 & 90.00 & 0.471 &0.296 & 75.00 & 0.501 &0.211 & 47.06 & 0.523 & 0.119 & 72.73 & 0.461 & 0.235 & 73.68\\
    \hdashline
   ChatGPT-4o&0.532 &0.782&80.00&0.507&0.615&75.00& 0.474&0.571&64.71&0.489&0.379&81.82&0.548&0.589&63.16\\
   Gemini Pro Vision&0.490&0.785&90.00&0.515&0.596&62.50&0.489&0.393&64.71&0.508&0.346&81.82&0.516&0.523&57.89\\
   Claude 3&0.290&0.733&80.00&0.492&0.536&75.00&0.414&0.448&64.71&0.280&0.317&81.82&0.490&0.557&57.89\\
   Grok &0.557 &0.835 &90.00&0.599&0.613&83.33&0.535&0.474&47.06&0.591&0.451&72.73&0.632&0.589&47.37\\ 
   \hline
   
   % *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.772} & \bf\blue{0.658}& 89.1 &\bf\blue{0.784} &0.825 &87.8 &\bf\blue{0.766} &\bf\blue{0.820}& 86.9 &\bf\blue{0.774} & \bf\blue{75.1} &\bf\blue{89.5} &\bf\blue{0.795} & 0.604 & \\
   % *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}&\\
   *InternVL3 (9B)~\cite{meta2024llama}&0.759&0.731&100.0&0.632&0.461&83.33&0.644&0.332&52.94& 0.623 &0.304&81.82&0.616&0.446&63.16\\
    *InternVideo2.5 (8B)&0.838&0.697&70.00&0.787&0.608&66.67&0.829&0.421&52.94&0.823&0.544&81.82&0.761&0.534&42.11\\
   \rowcolor{gray!20} \textbf{LOVE (Ours)}&0.862&0.850&100.0&0.759&0.672&83.33&0.814&0.553&70.59&0.837&0.574&81.82&0.792&0.663&73.68\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
  \vspace{-9mm}
%  \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
%     \toprule[1pt]
%      %\midrule
%      Dimension  &\multicolumn{3}{c}{\textbf{Single Class}}&\multicolumn{3}{c}{\textbf{Two Class}}&\multicolumn{3}{c}{\textbf{Counting}}&\multicolumn{3}{c}{\textbf{Colors}}&\multicolumn{3}{c}{\textbf{Position}}&\multicolumn{3}{c}{\textbf{Shapes}}\\
%   \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
%  Methods / Metrics
% &$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
%     \midrule
%      LLaVA-1.5 (7B)~\cite{liu2024improved} & 0.295  & 0.232 & 84.21 & 0.371  & 0.544 & 78.1 & 0.130 & 0.387 & 61.4 & 0.302  & 0.322 & 84.9 & 0.372 & 0.474 & 45.7 & 0.357 & 0.183   \\
%     LLaVA-NeXT (8B)~\cite{liu2024llavanext} & 0.393 & 0.244  & 83.5 & 0.459 & 0.451 & 79.1 & 0.319 & 0.460 & 68.42 & 0.308 & 0.424 & 83.5 & 0.434 & 0.408  & 46.3 & 0.403 & 0.433  \\
%     mPLUG-Owl3 (7B)~\cite{ye2024mplug} & 0.468 & 0.238  & 85.1 & 0.430 & 0.526 & 81.1 & 0.433 & 0.581 & 82.3 & 0.449 & 0.360 & 84.3 & 0.426 & 0.498  & 52.4 & 0.414 \\ 
%    MiniCPM-V2.6 (8B)~\cite{yao2024minicpm}& 0.423 & 0.350  & 85.1 & 0.311 & 0.697 & 77.9 & 0.361 & 0.711 & 83.9 & 0.353 & 0.547 & 85.5 & 0.445 & 0.607  & 55.56 & 0.45 \\
%     Qwen2-VL (7B)~\cite{Qwen2-VL} & 0.425 & 0.163  & 84.4 & 0.200 & 0.673 & 79.1 & 0.314 & 0.697 & 78.2 & 0.357 & 0.441 & 84.1 & 0.224 & 0.552  & 59.7 & 0.265\\
%      Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.507  & 0.394 & 18.6 & 0.495  & 0.716 & 44.6 & 0.493 & 0.705 & 53.0 & 0.524  & 0.505 & 21.9 & 0.569 & 0.648 & 74.9 & 0.602  \\
%     Llama3.2-Vision~\cite{meta2024llama}
%     &0.265&0.275&85.1&0.197&0.185&73.68&0.402&0.284&73.6&0.213&0.316 &87.9&0.233&0.154&48.9&0.252&0.301\\
%     DeepseekVL (7B)~\cite{lu2024deepseekvl}&0.137&0.043&82.5&0.192&0.447&74.07&0.222&0.194&78.9&0.094&0.134&80.3&0.275&0.332 \\
%     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.140 &0.032 &18.6 &0.157 &0.051 &44.6 &0.035 &0.028&53.0 &0.070 &0.046 &21.9 &0.048 &0.049 &74.9 &0.136 &0.03 \\
%     % DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1875 &0.0224 &0.4406 &0.2191 &0.0916 &0.4495 &0.2312 &0.0164&0.5545 &0.1640 &0.0824 &0.3260 &0.1701 &0.0555 &0.4757 &0.3304 &0.0453 &0.5050 & 0.2160 & 0.0549 & 0.5781\\
%   CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.341 & 0.316  & 85.3 & 0.292 & 0.536 & 81.3 & 0.319 & 0.389 & 71.1 & 0.433 & 0.378 & 84.3 & 0.407 & 0.410  & 35.2 & 0.492   \\
%   % InternVL2 (8B)~\cite{wang2024mpo}& 0.1230 & 0.3695  & 0.8345 & 0.1447 & 0.6436 & 0.8229 & 0.0701 & 0.5815 & 0.7136 & 0.0890 & 0.5478 & 0.8652 & 0.1585 & 0.6041  & 0.5412 & 0.0982 & 0.4042 & 0.6393 & 0.1226 & 0.5715 & 0.7232\\
%     InternVL2.5 (8B)~\cite{chen2024expanding}& 0.233  & 0.225 & 83.5 & 0.253  & 0.625 & 79.1 & 0.205 & 0.574 & 71.6 & 0.185  & 0.355 & 83.9 & 0.306 & 0.565 & 56.2 & 0.197 &   \\
%    InternLM-~\cite{internlmxcomposer}& 0.467 & 0.137  & 85.1 & 0.430 & 0.134 & 81.1 & 0.433 & 0.337 & 82.3 & 0.449 & 0.152 & 84.3 & 0.426 & 0.205  & 52.4 & 0.414 &  \\
%     % Llava-Onevision (0.5B)~\cite{li2024llava}& 0.1099 & 0.2670 & 0.7692 & 0.0068 & 0.3457 & 0.6057 & 0.0605 & 0.2331 & 0.7591 & 0.0460 & 0.1960 & 0.8571 & 0.0865 & 0.1988 & 0.7228 & 0.2047 & 0.2224 & 0.5871 & 0.0685 & 0.2074 & 0.6808\\
%    \hdashline
%    ChatGPT-4o\\
%    Gemini Pro Vision\\
%    Claude 3\\
   
%    *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.772} & \bf\blue{0.658}& 89.1 &\bf\blue{0.784} &0.825 &87.8 &\bf\blue{0.766} &\bf\blue{0.820}& 86.9 &\bf\blue{0.774} & \bf\blue{75.1} &\bf\blue{89.5} &\bf\blue{0.795} & 0.604 & 84.8&\bf\blue{0.799}  &0.604\\
%    *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& 0.708  & 0.609 & \bf\blue{89.5} & 0.705  & \bf\blue{0.828} & \bf\blue{89.2} & 0.699& 0.763 & \bf\blue{87.4} & 0.681  & 0.661 & 89.2 & 0.690& \bf\blue{0.777} & \bf\blue{88.3} & 0.725 & \bf\blue{0.788} \\
%    *Llama3.2-Vision (11B)~\cite{meta2024llama}& 0.734& 0.613& 72.6\\
   
%    \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.850}&\bf{\red{0.799}}&\bf\red{89.5}&\bf\red{0.861}&\bf\red{0.899}&\bf\red{89.3}&\bf\red{0.868}&\bf\red{0.867}&\bf\red{87.5}&\bf\red{0.860}&\bf\red{0.826}&\bf\red{89.5}&\bf\red{0.851}&\bf\red{0.841}&\bf\red{88.8}&\bf\red{0.863}\\
%    %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
%     \bottomrule[1pt]
%   \end{tabular}}
%   \vspace{0.6mm}
%     \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
%     \toprule[1pt]
%      %\midrule
%      Dimension  &\multicolumn{3}{c}{\textbf{Scene}}&\multicolumn{3}{c}{\textbf{Style}}&\multicolumn{3}{c}{\textbf{OCR}}&\multicolumn{3}{c}{\textbf{HOI}}&\multicolumn{3}{c}{\textbf{Human}}&\multicolumn{3}{c}{\textbf{Emotion}}&\multicolumn{3}{c}{\textbf{Linguistic Structure}}\\
%   \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\cmidrule(lr){20-22}
%  Methods / Metrics
% &$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
%     \midrule
%      LLaVA-1.5 (7B)~\cite{liu2024improved}& 0.337  & 0.298 & 92.2 & 0.445  & 0.209 & 74.0 & 0.454 & 0.666 & 83.4 & 0.457  & 0.428 & 71.8 & 0.447 & 0.428 & 83.9 & 0.288 & 0.423 & 63.4 & 0.427 & 0.278 & 77.2 \\
%     LLaVA-NeXT (8B)~\cite{liu2024llavanext}& 0.517 & 0.336  & 87.3 & 0.502 & 0.326 & 77.6 & 0.560 & 0.629 & 92.6 & 0.521 & 0.596 & 75.8 & 0.486 & 0.310  & 85.3 & 0.444 & 0.502 & 55.9 & 0.565 & 0.565 & 80.7 \\
%     mPLUG-Owl3 (7B)~\cite{ye2024mplug}& 0.448 & 0.013 & 87.3 & 0.209 & 0.202 & 76.7 & 0.361 & 0.669 & 86.0 & 0.460 & 0.498 & 75.3 & 0.460 & 0.443  & 83.2 & 0.333 & 0.500 & 62.9 & 0.499 & 0.555 & 84.6 \\ 
%        MiniCPM-V2.6 (8B)~\cite{yao2024minicpm}& 0.369 & 0.126  & 87.3 & 0.475 & 0.467 & 77.6 & 0.525 & 0.727 & 85.6 & 0.403 & 0.545 & 74.6 & 0.450 & 0.478  & 85.7 & 0.313 & 0.515 & 64.1 & 0.436 & 0.657 & 82.5\\
%     Qwen2-VL (7B)~\cite{Qwen2-VL}& 0.398 & 0.297  & 87.7 & 0.525 & 0.439 & 75.6 & 0.511 & 0.720 & 92.1 & 0.293 & 0.567 & 75.1 & 0.250 & 0.574  & 82.6 & 0.417 & 0.574 & 62.3 & 0.485 & 0.693 & 82.5\\
%      Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& 0.548  & 0.435 & 91.9 & 0.537  & 0.424 & 74.4 & 0.658 & 0.773 & 90.4 & 0.519  & 0.543 & 77.1 & 0.560 & 0.454 & 80.1 & 0.441 & 0.493 & 51.0 & 0.610 & 0.701 & 84.4\\
%     Llama3.2-~\cite{meta2024llama}
%     &0.355&0.047&92.2&0.409&0.342&75.1&0.178&0.258&88.8&0.277&0.086 &72.3&0.196&0.162&69.2& 0.237& 0.128& 59.0& 0.322 &0.442 &59.0\\
%     DeepseekVL (7B)~\cite{lu2024deepseekvl}
%     &0.333&0.109&89.0&0.301&0.012&75.8&0.352&0.199&74.2&0.360&0.286&70.37&0.456&0.141&78.5&0.249&0.330&66.0&0.444&0.502&83.9 \\ 
%     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.140 &0.031 &16.9 &0.157 &0.006 &26.3 &0.070 &0.067&68.1 &0.048 &0.015 &31.4 &0.136 &0.029 &32.5 &0.078 &0.057 &33.7&0.257 &0.013 &76.5\\
%     % DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.3410 &0.0226 &0.7175 &0.3403 &0.0464 &0.5457 &0.4329 &0.1551 &0.2620 &0.3279 &0.0198 &0.4938 &0.2298 &0.0187 &0.7246 &0.1676 &0.0112 &0.3568 & 0.4062 & 0.0420 & 0.5897\\
%   CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.357 & 0.024  & 87.3 & 0.586 & 0.252 & 77.4 & 0.493 & 0.383 & 65.1 & 0.460 & 0.307 & 71.6 & 0.356 & 0.163  & 80.3 & 0.298 & 0.256 & 61.6 & 0.482 & 0.404 & 83.0 \\
%     % InternVL2(8B)~\cite{wang2024mpo} & 0.1899 & 0.1946  & 0.8734 & 0.4383 & 0.5235 & 0.7237 & 0.2537 & 0.6595 & 0.8515 & 0.2062 & 0.4766 & 0.7506 & 0.0633 & 0.4308  & 0.8613 & 0.1378 & 0.4761 & 0.5117 & 0.3134 & 0.6197 & 0.8042\\
%     InternVL2.5 (8B)~\cite{chen2024expanding}& 0.218  & 0.216 & 89.9 & 0.344  & 0.406 & 74.4 & 0.349 & 0.666 & 72.1 & 0.355  & 0.473 & 73.6 & 0.249 & 0.446 & 82.0 & 0.237 & 0.517 & 58.2 & 0.357 & 0.613 & 74.6 \\
%    InternLM~\cite{internlmxcomposer}& 0.448 & 0.034 & 87.3 & 0.209 & 0.026 & 76.7 & 0.361 & 0.060 & 86.0 & 0.460 & 0.275 & 75.3 & 0.460 & 0.080  & 83.2 & 0.333 & 0.157 & 62.9 & 0.499 & 0.346 & 84.6\\
%     % Llava-Onevision(0.5B)~\cite{li2024llava}& 0.1844 & 0.3412 & 0.8766 & 0.2037  & 0.3358 & 0.6164 & 0.2900 & 0.0586 & 0.7598 & 0.0210 & 0.2987 & 0.5636 & 0.0430 & 0.3270 & 0.2153 & 0.1076 & 0.3139 & 0.6270 & 0.1655 & 0.0327 & 0.7646\\
%    \hline
%    *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.763} & \bf\blue{0.591}& 93.2 &\bf\blue{0.730} &\bf\blue{0.677} & \bf\blue{83.8} &0.855 &0.825& 91.2 &\bf\blue{0.800} & \bf\blue{0.667} & 80.3 &\bf\blue{0.846} & \bf\blue{0.719} & 88.4 &\bf\blue{0.790}  &0.670& 79.8 &\bf\blue{0.812} &0.375& 87.2\\
%    *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& 0.680  & 0.521 & \bf\blue{93.2} & 0.668  & 0.642 & 83.7 & \bf\blue{0.881}& \bf\blue{0.850} & \bf\blue{92.9} & 0.751  & 0.611 & \bf\blue{83.5} & 0.693& 0.562 & \bf\blue{92.0} & 0.633 & \bf\blue{0.690} & \bf\blue{82.9} & 0.754 & \bf\blue{0.795} & \bf\blue{88.3}\\
%     *Llama3.2-Vision (11B)~\cite{meta2024llama}&0.760 & 0.456& 92.5& 0.720& 0.481& 78.95&0.842 &0.526&80.4&0.790 & 0.469& 74.6&0.817 & 0.635& 84.5&0.759 & 0.463&77.5&0.801& 0.273&73.68\\
%    %\hdashline
%    \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.856}&\bf{\red{0.755}}&\bf\red{93.3}&\bf\red{0.860}&\bf\red{0.804}&\bf\red{86.1}&\bf\red{0.938}&\bf\red{0.882}&\bf\red{93.0}&\bf\red{0.921}&\bf\red{0.864}&\bf\red{83.5}&\bf\red{0.916}&\bf\red{0.851}&\bf\red{92.0}&\bf\red{0.907}&\bf\red{0.864}&\bf\red{84.7}&\bf\red{0.878}&\bf\red{0.837}&\bf\red{88.4}\\
%    %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
%     \bottomrule[1pt]
%   \end{tabular}}
  
%   \vspace{0.6mm}
%       \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
%     \toprule[1pt]
%      %\midrule
%      Dimension  &\multicolumn{3}{c}{\textbf{View}}&\multicolumn{3}{c}{\textbf{World Knowledge}}&\multicolumn{3}{c}{\textbf{Face}}&\multicolumn{3}{c}{\textbf{Imagination}}&\multicolumn{3}{c}{\textbf{Time \& Light}}&\multicolumn{3}{c}{\textbf{Complex}}&\multicolumn{3}{c}{\textbf{Overall}}\\
%   \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\cmidrule(lr){20-22}
%  Methods / Metrics
% &$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$&$\rho_p$$\uparrow$&$\rho_c$$\uparrow$&Acc$\uparrow$\\
%     \midrule
%      LLaVA-1.5 (7B)~\cite{liu2024improved}& 0.389  & 0.255 & 73.6 & 0.309  & 0.450 & 80.1 & 0.401 & 0.375 & 65.6 & 0.395  & 0.504 & 68.42 & 0.396 & 0.413 & 73.1 & 0.336 & 0.471 & 66.3 & 0.337 & 0.389 & 71.0 \\
%     LLaVA-NeXT (8B)~\cite{liu2024llavanext}& 0.534 & 0.284  & 70.5 & 0.522 & 0.313 & 84.7 & 0.475 & 0.438 & 64.71 & 0.579 & 0.568 & 69.0 & 0.504 & 0.448  & 70.5 & 0.403 & 0.413 & 59.7 & 0.433 & 0.457 & 70.7\\
%     mPLUG-Owl3 (7B)~\cite{ye2024mplug}& 0.448 & 0.399  & 71.3 & 0.458 & 0.369 & 80.3 & 0.077 & 0.340 & 68.0 & 0.354 & 0.493 & 66.8 & 0.385 & 0.539  & 69.2 & 0.402 & 0.517 & 64.71 & 0.392 & 0.474 & 72.73 \\ 
%    MiniCPM-V2.6 (8B)~\cite{yao2024minicpm} & 0.407 & 0.404  & 76.1 & 0.382 & 0.468 & 61.7 & 0.323 & 0.510 & 70.7 & 0.475 & 0.625 & 71.5 & 0.451 & 0.464  & 65.7 & 0.333 & 0.538 & 66.1 & 0.373 & 0.592 & 73.4\\
%     Qwen2-VL (7B)~\cite{Qwen2-VL} & 0.518 & 0.488  & 77.1 & 0.590 & 0.540 & 79.7 & 0.492 & 0.577 & 69.1 & 0.385 & 0.581 & 67.9 & 0.517 & 0.543  & 67.4 & 0.350 & 0.605 & 62.2 & 0.376 & 0.590 & 72.6\\
%      Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& 0.537  & 0.457 & 76.1 & 0.562  & 0.496 & 70.5 & 0.626 & 0.549 & 72.1 & 0.598  & 0.602 & 72.6 & 0.556 & 0.504 & 66.67 & 0.549 & 0.685 & 74.7 & 0.528 & 0.640 & 76.2\\
%     Llama3.2-~\cite{meta2024llama}
%     &0.311&0.146&73.0&0.235&0.140&66.4&0.274&0.087&71.3&0.233&0.227 &70.4&0.370&0.130&61.5&0.284&0.155&60.9&0.293&0.260&70.8\\
%     DeepseekVL (7B)~\cite{lu2024deepseekvl}
%     &0.357&0.228&70.1&0.355&0.233&76.7&0.293&0.177&65.2&0.311&0.502&70.1&0.400&0.252&67.8&0.205&0.325&56.8&0.261&0.236&70.7 \\ 
%     DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.200 &0.084 &30.5 &0.175&0.013 &16.9&0.168 &0.039 & 41.18 &0.172 &0.021 &39.8 &0.179 &0.001 &33.9 &0.048 &0.015 &62.2 &0.125 &0.032 &42.7\\
%     % DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.2916 &0.0569 &0.4371 &0.2757 &0.1169 &0.2349 &0.3585 &0.0913 &0.5117 &0.2294 &0.1188 &0.5109 &0.4237 &0.0011 &0.5271 &0.2140 &0.0226 &0.5353 & 0.2577 & 0.0404 & 0.4921\\
%   CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.349 & 0.308  & 70.9 & 0.435 & 0.312 & 79.3 & 0.488 & 0.366 & 68.2 & 0.395 & 0.385 & 62.2 & 0.428 & 0.314  & 67.3 & 0.413 & 0.280 & 48.0 & 0.386 & 0.358 & 67.5 \\
%   % InternVL2(8B)~\cite{wang2024mpo}& 0.1341 & 0.4399  & 0.6825 & 0.2283 & 0.5327 & 0.7831 & 0.3015 & 0.3548 & 0.7031 & 0.2657 & 0.5622 & 0.7318 & 0.1645 & 0.3668  & 0.5833 & 0.1378 & 0.5257 & 0.6714 & 0.1492 & 0.5713 & 0.7198\\
%     InternVL2.5 (8B)~\cite{chen2024expanding}& 0.307  & 0.359 & 70.37 & 0.315  & 0.426 & 78.5 & 0.301 & 0.490 & 66.6 & 0.347  & 0.489 & 71.4 & 0.333 & 0.373 & 56.4 & 0.228 & 0.590 & 60.8 & 0.260 & 0.551 & 70.1 \\
%    InternLM~\cite{internlmxcomposer}& 0.448 & 0.227  & 71.3 & 0.458 & 0.205 & 80.3 & 0.077 & 0.113 & 68.0 & 0.354 & 0.188 & 66.8 & 0.385 & 0.020 & 69.2 & 0.402 & 0.170 & 64.71 & 0.392 & 0.173 & 72.73\\
%     % Llava-Onevision(0.5B)~\cite{li2024llava}& 0.120  & 0.117 & 0.736 & 0.152 & 0.273 & 0.297 & 0.301 & 0.313 & 0.596 & 0.014  & 0.455 & 0.429 & 0.207 & 0.215 & 0.386 & 0.038 & 0.138 & 0.659 & 0.119 & 0.249 & 0.618\\
%    \hline
%       *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.771} & 0.670&83.9 &\bf\blue{0.815} &0.678 & 89.8 &0.837 &\bf\blue{0.689}& 77.2&\bf\blue{0.767} & \bf\blue{0.764} & 81.82 &\bf\blue{0.771} & 0.666 & 82.6&\bf\blue{0.769}  &0.778 &83.7&\bf\blue{0.790} &0.782& 84.9\\
%       *Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}& 0.712  & \bf\blue{0.782} & \bf\blue{85.1} & 0.734  & \bf\blue{0.713} & \bf\blue{90.4} & 0.760& 0.648 & \bf\blue{82.2} & 0.594  & 0.736 & \bf\blue{88.0} & 0.707& \bf\blue{0.718} & \bf\blue{82.7} & 0.668 & \bf\blue{0.811} & \bf\blue{89.2} & 0.699 & \bf\blue{0.801} & \bf\blue{87.2}\\
%     *Llama3.2-Vision (11B)~\cite{meta2024llama}&0.718 & 0.258& 81.4& 0.759& 0.658& 88.0&\bf\blue{0.837} &0.598&77.3&0.723 & 0.624& 79.6&0.745 & 0.653& 82.2&0.714 & 0.532&75.9&0.756& 0.640&78.1 \\
%    %\hdashline
%    \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.870}&\bf{\red{0.814}}&\bf\red{85.0}&\bf\red{0.885}&\bf\red{0.814}&\bf\red{90.5}&\bf\red{0.949}&\bf\red{0.906}&\bf\red{82.4}&\bf\red{0.886}&\bf\red{0.882}&\bf\red{88.5}&\bf\red{0.878}&\bf\red{0.829}&\bf\red{83.0}&\bf\red{0.877}&\bf\red{0.901}&\bf\red{89.2}&\bf\red{0.886}&\bf\red{0.895}&\bf\red{87.9}\\
%    %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
%     \bottomrule[1pt]
%   \end{tabular}}
  \label{lmm}
  % \vspace{-1em}
\end{table*}
